Convolutional Visual Prompt for Robust Visual Perception

Vision models are often vulnerable to out-of-distribution (OOD) samples without adapting. While visual prompts offer a lightweight method of input-space adaptation for large-scale vision models, they rely on a high-dimensional additive vector and labeled data. This leads to overfitting when adapting models in a self-supervised test-time setting without labels. We introduce convolutional visual prompts (CVP) for label-free test-time adaptation for robust visual perception. The structured nature of CVP demands fewer trainable parameters, less than 1\% compared to standard visual prompts, combating overfitting. Extensive experiments and analysis on a wide variety of OOD visual perception tasks show that our approach is effective, improving robustness by up to 5.87% over several large-scale models.

==> docs/rebuttal.tex <==


We are very grateful to Reviewers uZKT (\RI), zs9s (\RII), HEpT (\RIII), XDjm (\RIIII) and QKSZ (\RIIIII) for your efforts in reviewing our paper and for your many insightful questions and helpful suggestions. We are delighted and humbled to receive unanimously positive feedback from the reviewers:

- The paper proposes a novel, well-motivated and would interests the visual prompt community.
- Extensive experiments have been conducted across a variety of OOD recognition. The main and ablation experiments are large-scale.
- The paper is well-written and comprehensible, offering clear explanations.

We fully response and address all the questions that the reviewers asked and includes additional experiments, figures to support ours responses. We will definitely add all the details into our later revision.  The figures and tables can be found in the PDF file. 

Sorry for the missing details which cause some misunderstanding to Reviwer QKSZ (\RIIII), we will add all details into our supplementary in the later revision.

Thank you again for your efficient handling of our submission.

\section{Review uZKT}

\subsection{Motivation of using convolutional visual prompt for test-time adaptation}

%  What motivated the choice of convolutional structures over other possible structures for the CVP?
% Thanks to the reviewer for all the great suggestions. We agree with the reviewer that our CVP can be viewed as a de-corruption operator for natural images. Moreover, we empirically discovered the OOD samples could damage the SSL objectives, such as the contrastive learning, and show the shifting of loss variances in Figure 2.  Motivated by these two insights, we choose the CVP modules with SSL tasks to adapt the OOD samples.

%cz version
Thank you for your question. We agree with the reviewer that our CVP can be viewed as a de-corruption operator for natural images. Our paper studies how to be robust under major natural distribution shifts, such as style, smoothness, or lightening changes. Those shifts are often locally structured, which motivates us to use convolution that handles locally structured data. Empirically, our convolution directly undo the corruption, as shown in Figure 11.
Moreover, our empirical results show that our proposed convolutional visual prompts outperform standard visual prompts and low-rank visual prompts. We will make the input de-corruption operation point more clear in our revision.
It will be interesting to explore how well CVP adapts to more global changes, such as shape change, which we leave for future work.

% The corruption is structured so convolution is a good way to reverse the corruption
% Convolution are designed to operate on locally change, A large portion of corruption like blurring are locally structured and can be recovered by convolution
% Without convolution kernel, it is less effective, motivate us to use the convolution


\subsection{Discuss the wider usage of CVP when applied to settings other than test-time adaptation}

We thank the reviewer for pointing out this. We will add it in the discussion part for the later revision. We list a few additional usages of CVP bellow:

1. Beyond unsupervised test-time adaptation, we can also supervisedly optimize our convolutional visual prompt when a few labeled data are available on the target domain. Since our convolutional visual prompt has fewer parameters, applying it to this setting can reduce the training cost. 

2. Continual learning can benefit from our lightweight CVP. Since the environment often changes incrementally, applying the structured CVP adaptation can potentially help continual adaptation without forgetting.

3. The model deployed on edge devices can also benefit from CVP. As it has limited memory and requires handling multiple types of corruption, the efficiency of the parameter of CVP allows us to maintain individual prompts for each scenario without using too much memory. 


\subsection{Discuss the extendability of CVP model}

Thank you for your question. Yes, our method can be extended by stacking deeper convolutional prompts. In addition, future work can study adding CVP to the latent representations and study if the hyper network can be used to generate the parameters for the CVP for meta-learning. In terms of application, CVP can be used to adapt not only classification models but also generative models such as diffusion. 


\section{Review zs9s}

\subsection{Novelty of our work}

Our paper provides deep insights on what is a good visual prompt design for test-time adaptation, which is an important problem. The key novelty of our work is to propose this simple and effective convolutional visual prompt to address the overfitting challenge at test time.
Prior work like convolutional residual adapter adapts the model architecture with lots of parameters, which is designed for training time optimization but can lead to overfitting on test-time adaptation. Our method only adds a small convolutional prompt on the inputs during the inference time, which is both lightweight and avoids test-time overfitting.
Moreover, the other Reviewers XDjm and HEpT find our method to be novel and well-motivated. Reviewer uZKT also mentions this research direction would interest the visual prompt community.

\subsection{Performance compared with other methods ( BN [53] and TENT [60])}

our method is orthogonal to BN [53], TENT [60] and can be applied on top of them, improving those methods even more. 

Since our method updates only the input prompt without modifying the model weights, it works with frozen models and avoids the high cost of fine-tuning (especially on edge devices like smartphones). 

Our work provides a new direction for the robustness field by visual prompting at test time, which we think is worth publishing.

% Our CVP is orthogonal to [53] [60], where we focus on a harder scenario: the model weights can not be adjusted during the inference time. As shown in Tables 1, 2, and 3, CVP outperforms other input-weight adaption baselines.

% BN [53] and TENT [60] require changing the model weights during test time which is unrealistic. Therefore, in Table 4., we show our CVP has additional improvements on top of BN [53] and TENT [60] even under the setting that model weights can be adjusted.


\subsection{Compare with relevant baselines such as [1]}

We thank the reviewer for suggesting this relevant paper, which we will cite. 

We highlight the difference between our work and this paper as follows. 1.) Our CVP creates during the adaptation phase, and we don't need any source domain sample to tune the prompt first. 2.)  In contrast to [1] tuning a collection of visual prompts and the classification head, we adapt every batch sample using CVP, which is just a single convolutional kernel. Our method is simple, lightweight, and easy to use.

[1] Gao, Yunhe, et al. "Visual prompt tuning for test-time domain adaptation." arXiv preprint arXiv:2210.04831 (2022).

\subsection{Comparison to / on top of UDG baselines that solve the same problem}

Standard UDG methods require training on multiple source domains and testing generalization on a different domain, which is not the ImageNet benchmark setup we evaluate on. 
Our UDG scenario has only a single training domain, like Imagenet, and tests the model on multiple OOD domains. We thus only compare UDG methods that conduct single-domain training, such as BN, TENT, MEMO. Experimenting with UDG with multiple training domains is out of the scope of our paper. We would like to include more baselines if the reviewer can point out other single training domains UDG work that we are missing.

\subsection{Combining other methods}
Thank you for your question. We agree that since our method applied a prompt for the input, it can be easily combined with other methods that change the model weights. We believe our method can further improve the robustness of future work that adapts model weights.


\subsection{Supervised variant of the approach.}
Sorry for the confusion. We want to clarify that results from the supervised variant are only for training the best case and thresholding the upper bounds of our method. The main contribution of our paper is to apply the unsupervised variant on test-time adaptation. 

% While our method can be applied to supervised learning, it is not the claim of the paper. mention supervised is upper bound

% We will remove the supervised variant and make our studied problem more clear in our revision.



% Our goal is to focus on test-time adaptation without the annotations, where we indeed compare with the transductive few-shot method (For example: MEMO) under the self-supervised setting (see Table 4.). The supervised variant of the approach represents the baseline which is not our main contribution. 


\subsection{The online test-time tuning with one sample.}

Our convolutional visual prompt is general and can be applied to other SSL tasks that use one sample. In Table 7, we show our method also works with rotation prediction and MAE, which only needs one sample and achieves up to 3.14\% improvement in robustness. 
We will cla....

\subsection{Can CVP complement other parameter-efficient tuning (PEFT) methods?}

Yes, they are complementary. The PEFT methods often update the model weights, while our CVP updates the input. Thus our method is orthogonal to PEFT and can be directly applied to PEFT to further improve the model adaptation performance.

% In the following Table, we run the CVP + prefix tuning and compare with prefix tuning only, where we add the prompt into the latent features and try to optimize them with SSL loss. As the results show, ... The CVP + prefix tuning does not improve because PEFT provides a huge capability to adapt the model and lead to overfit for adaptation.
% In the later revision, we will add the experiments on other benchmarks under this setting.


% |                | s1    | s2    | s3    | s4    | s5    |

% |----------------|-------|-------|-------|-------|-------|

% | Standard       | 59.68 | 47.88 | 40.31 | 32.75 | 28.20 |

% | CVP + prefix tuning | 62.17 | 49.94 | 41.49 | 33.72 | 28.35 |


[1] Visual prompt tuning for test-time adaption


\section{Review HEpT}
We appreciate the reviewer’s comments and suggestions. Thanks to the reviewer for recognizing the novelty of our work. We have answered and addressed the questions.

\subsection{Comparison with other prompts.}

Thank you for your suggestion in comparing with other prompts. We follow your suggestion and include additional comparison with shallow prompt [26], in the Table below. explain the number...
We would like to mention that [A] uses text prompts that is tailored to vision language model adaptation. Ours method is more general and can be applied to any visual perception model.


|                | s1    | s2    | s3    | s4    | s5    |
|----------------|-------|-------|-------|-------|-------|
| CLIP-ViT-b/32  | 58.58 | 48.45 | 40.12 | 33.38 | 27.51 |
| Shallow prompt [26] | 56.87 | 47.22 | 38.72 | 30.49 | 24.10 |  
| CVP            | 59.11 | 49.09 | 40.76 | 33.51 | 27.80 |




% Our method adapts the prompt at test time. Since no ground truth label is available, the existing training time prompt method does not work. We include the results of a few popular prompts methods, such as the shallow prompt shown in [26]. We extract the latent features from the vision encoder and append the prompt for tuning. We set up the same tuning method, which uses the self-supervised objective to adapt the sample. The following shows our results. 
% The Shallow prompt does not improve under our setting because it requires more learnable parameters in the prompt and leads to overfitting for adaptation.



% We believe our CVP method can be combined with text prompt tuning, yet it is currently out of our scope. We will add it in our later revision.


\subsection{Other test-time adaption method.}

% The paper mentions on L63: “The only one that does not update the model (for Test time adaptation) is proposed by [40]”. However the following uncited works do not update the model as well [A, B].

[todo] mention the difference between ours and related works

We thank the reviewer for pointing out those works [A] [B]. We will cite them in our revision.

[A] Test-Time Prompt Tuning for Zero-Shot Generalization in Vision-Language Models. Shu et al.
[B] Test-Time Training with Masked Autoencoders. Yossi et al.

\subsection{ViT Results
}
Thank the reviewer for suggesting this. We run the experiment for CVP on the ViT-Base model and show a similar gain in performance.
The following table shows our results of the ViT-Base model for 15 types of corruption under severity level 1 on CIFAR-10-C. The test accuracy of ViT-Base clean CIFAR10 is 96.42\%. Compared to the accuracy (\%) before adaptation (standard) and using VP to do the adaptation, the CVP achieves better performance up to 2 points.


|                   |          | ViT-BASE |       |
|-------------------|----------|:--------:|-------|
|                   | standard |    VP    |  CVP  |
|      Gaussian     |   47.64  |   49.71  | 50.22 |
|        Shot       |   41.92  |   45.67  | 46.03 |
|      Impulse      |   80.77  |   80.39  | 82.13 |
|    Defocus blur   |   27.91  |   27.37  | 28.90 |
|    Motion blur    |   58.34  |   56.22  | 58.87 |
|     Glass blur    |   48.49  |   47.77  | 49.12 |
|     Zoom blur     |   83.71  |   83.23  | 85.63 |
|     Brightness    |   94.40  |   93.10  | 94.59 |
|        Fog        |   74.75  |   73.60  | 75.63 |
|       Snow        |   89.37  |   88.23  | 89.41 |
|       Frost       |   90.13  |   92.19  | 92.32 |
|      Contrast     |   90.14  |   91.34  | 92.34 |
| Elastic Transform |   40.68  |   40.52  | 41.52 |
|  JPEG compression |   62.53  |   61.55  | 63.53 |
|      Pixelate     |   66.06  |   66.37  | 66.35 |
| Averaged Acc. | 66.45 | 66.48 | **67.77** |

\subsection{The choice of hyper-parameter setting on kernel size and lambda range} 

$\bullet$ For the lambda parameter, it controls the magnitude of convolved output when combined with the residual input. We set the lambda range to be [0.5, 3] and run test-time optimization to automatically find the optimal solution, which does not require a validation set. 

$\bullet$ We use 3x3 for cifar-10 and 5x5 for ImageNet. In general, small kernel size is used to avoid overfitting. We increase the kernel size for large images, such as ImageNet.

$\bullet$ For the update iterations, as the Table 17. show a larger number of iterations has better performance. However, the training cost becomes higher.

\subsection{Missing details on evaluation and implementation}

- Thanks for mentioning it. We will add all of these details in our later revision.

\subsubsection{What hyperparameters are used in Table 4/5/7, where the kernel size is not specified}

$\bullet$  For Table 4, we set the kernel size for CIFAR-10-C as 3*3 and ImageNet-C, R, S, and A as 5*5. The adaptation iterations are all set as 5.

$\bullet$  For Table 5, same as the setting above, the CIFAR-10-C uses the 3*3 and others use 5*5. The adaptation iterations are all set as 5.

$\bullet$  For Table 7, we evaluate the performance for three SSL tasks on ImageNet-C. The standard model is ResNet50. For the CVP kernel, we use the same setting as above, the 5*5, which is the optimal choice. 

\subsubsection{How is CVP applied to CLIP-ViTs? Is the image first convolved and then tokenized?}

$\bullet$ Sorry for missing detail. Yes, our CVP is applied before tokenized. The CVP is applied to CLIP-ViTs by adding a convolutional kernel on the input sample and then getting an adapted sample as a new input iteratively. We will add more detail on how CVP applies to CLIP in our later revision. 

\subsubsection{Which CLIP-ViT/32 model and can was used for the results in Table 3?}

$\bullet$ Thanks for the careful check. The CLIP model we use for evaluation is the CLIP-ViT-base/32. In our later revision, We will clarify our model CLIP-ViT/32 as CLIP-ViT-base/32.

\subsubsection{What architecture is used for the results in Table 7?}

$\bullet$ The architecture we use for Table 7 is the ResNet50 pre trained with original ImageNet-C.

\subsubsection{Clarification for MAE baseline.}

Yes,  the contrastive objective of CVP is directly replaced by MAE objective. We replace the contrastive loss as reconstruction loss.
Since the decoder for MAE is fixed, we do not optimize additional parameters at test-time adaptation.

% $\bullet$ No, we do not add additional trainable parameters here. As the d, we only require the reconstruction loss to optimize the convolutional kernels' parameters. The parameters for three different SSL tasks are the same.

\subsubsection{L9: 1\% when compared to standard visual prompts”. How does this compare to the shallow prompts used in}

Thank you for your question. We compared to shallow prmopts which is also less than 1\%.

% $\bullet$ While our method focuses on input-based prompts, shallow prompts are not in our current scope. Therefore, the standard visual prompts in L9 indicate the "input-based prompts". Here, we add the results for shallow prompt under our SSL setting. We also show the comparison of a number of parameters.

% |                | s1    | s2    | s3    | s4    | s5    |

% |----------------|-------|-------|-------|-------|-------|

% | Standard       | 59.68 | 47.88 | 40.31 | 32.75 | 28.20 |

% | shallow prompt | 62.17 | 49.94 | 41.49 | 33.72 | 28.35 |

% | CVP            | 69.07 | 54.73 | 45.96 | 37.79 | 31.61 |

\subsubsection{Why CVP doesn't outperform baseline on weather conditions}
While our CVP doesn't outperform the VP baseline on weather corruption, it actually outperforms the results of the standard baseline. In Figure 2., we show deep insight into the contrastive loss distribution and empirically find that the weather corruption (for example: snow) leads to a huge shift from the source domain even in the low severity. Therefore, we conjecture that the weather corruption types over-damaged the intrinsic structure and need more learnable parameters to restore the structure back.

\subsubsection{In Table 15, are the reported losses on samples that were used to tune prompts?}

Yes, we report the losses for samples already tuning with the prompt. 

\subsection{Reporting the loss on unseen samples }

--  We run the unseen test sample loss to show the avoid of overfitting.

![image info](./figs/unseen_loss_analysis.png width="50")


\subsection{Dual text-visual prompt tuning (like [C]) with: CVP (your method) + [A] (NeurIPS’22)}

Thank you for these suggestions. We feel that combining text prompts and CVP is an interesting idea. We will add it in future work.




\section{Review XDjm}

Thank you for endorsing and recognizing our work as realistic, interesting, and well-studied.

\subsection{CVP would still work well for high-level distribution shift, such as style changes?}

It's a very good point. We do have experiments on those style changes benchmark such as the ImageNet-Rendition, Sketch, and Adversarial. Our results show that CVP can improve robust accuracy on such a high-level distribution shift.

\subsection{In L206., "starting from a sharpness kernel is effective". Could the authors elaborate on what 'sharpness kernel' is and why it is effective?}

When adapting, the kernel should be initialized with fix/random initialization. We use a sharpness kernel as an initial point for the fixed initialization setting, which is a n*n matrix. It starts from specific values, which can control the edge enhancement effect by extracting the frequency information of inputs with a high pass filter. When the kernel size is 3, we set up the sharpness kernel as [[0,-1, 0], [-1, 5, -1], [0, -1, 0]]
Similar to the convolutional kernel prompt, sharpness transforms an image using a convolutional 2D filter. It simultaneously enlarges the high-frequency part of images and then filters the low frequencies part.



\subsection{Can convolutional kernel applies on the partial region}
This is an interesting point. We only apply it to the whole image. We will study this in future work.


\section{Review QKSZ}

\subsection{Clarification for contrastive formulation.}

The loss indeed considers the negative pair, which is in the denominator. If $x_{i}$ and $x_{j}$ are positive pair, the $y_{i,j}$ is 1; then we maximize the similarity between the pos on the nominator and minimize the denominator, which is similarity between all negative pairs $x_{i}$ and $x{k}$, where $j \neq k$. When $y_{i,j}$ is zero, the whole term is 0, and does not impact the loss.

\subsection{Clarification for test-time adaptation framework}

TODO: find a citation 

As the paper[1] defined, Test-time adaptation as running optimization at test time for target-domain data, which does not prohibit a model pre-trained with source data [1]. Test-time adaptation methods, such as TENT, TTT, MEMO, all train their model using the source data. 

[1] VISUAL PROMPT TUNING FOR TEST-TIME DOMAIN
ADAPTATION

% , where the backbone classifier are all first trained on source domain data. We simply use the same source domain data to train an additional self-supervised task, like TTT, which does not require any additional data than what the backbone classifier has been trained on.

% - Our method is indeed a test-time adaptation framework, as we only allow access to the target domain data and do the one-time adaption during the test time.
% We want to clarify the definition of test-time adaptation. The TTA means we adapt the OOD samples during the test time without any source domain information. 

\subsection{What tells that the distribution shift is 'visually structured'?}

Our visual world is known to be structured, and the changes are not random. For example, when weather starts to rain, the shift introduced by rain is highly structured, you can tell there is rain in the image. This is our assumption about the visual world, which works well according to our empirical results. We agree that our method cannot handle arbitrary shifts that are not structured, which is out of the scope of our paper.

% We have shown the attention visualization in Figure 5 and 11, which gives us the insight that the distribution shift is visually structured. Besides, Figure 2 shows the huge change on loss distribution for different corruption types.

\subsection{Clarification Line 180**}

$\bullet$ The conv. operation is applied to the image and only during the adaptation phase. We draw the model architecture in pdf Figure .  TODO

$\bullet$ Yes, MLP is used for inference. But it is fixed during inference. Figure 6 shows the number of learnable parameters at test time. 



**Question on proposed method**

- There are two phases in our proposed method. The first one is to do the offline one-time training on SSL. The second one is the online test-time adaption for any OOD benchmark.
- The training of the SSL model is offline training with a simple MLP architecture. We don't require the conv operation for training it, yet we only use the latent representation extracted from the logit layer of the backbone model to train this SSL with the original ImageNet dataset. During the inference time, the MLP can be used to extract the features for calculating the contrastive loss.
- The Conv operation is only used during the test-time adaption. We apply it to every upcoming batch and adapt them in several iterations. 
As the comparison of learnable parameters is on test-time adaptation only, we don't take into account the learning of SSL.

[todo] draw the num. of learnable prams.
**Missing X-axis**

- Sorry for the confusion. We replot the figure again. The x-axis is in the unit K.

\subsubsection{Line 184: extension to CLIP}

we focus on the convolutional prompt that is only applicable to the vision encoder. We will study how to combine text prompts with CVP in future works.

\subsubsection{Clarification: Section 4.1 FT and PFT Baseline}

Yes. Current test-time adaptation initial or reset the weights after one-time adaptation. We choose this experiment setup because the samples usually come by batch, and the batch is not correlated with the prior one.

\subsubsection{Line 206: What is a sharpness kernel?}
The sharpness kernel is a n*n kernel starting from specific values which can control edge enhancement effect by extracting the frequency information of inputs with a high pass filter. 
Similar to the convolutional kernel prompt, sharpness transforms an image using a convolutional 2D filter. It simultaneously enlarges the high-frequency part of images and then filters the low frequencies part.

\subsubsection{Compared to standalone CVP, CVP+x provides a huge error rate drop - then this means the major workforce behind the performance is x and not CVP.}

Our main contribution is to study and propose CVP, an input adaptation method that is orthogonal to those adaption methods such as BN, TENT, or MEMO. Unlike their method requires to adjust the model weight, ours is more efficient and only requires 1\% less of learn-able parameters than theirs. Therefore, we show how CVP can improve the robust accuracy on top of them.

\subsubsection{More details about low-rank prompts}

-- Pseudo algorithm:

-- SVD on input X (N*C*H*W) →  get n pairs of initial $ U \Sigma V^T$  (3 channel)

-- Set rank number R (ex: 3)

-- For every adapt iteration t:

-- Get N inverse matrices $M_t = U_t x \Sigma_t x VT _t$ 

-- Apply low rank SVD on $M_t$ with rank ‘R’ —> get low $rank U’_t, \Sigma’_t, V’T _t$

-- $M’_t = U’_t x \Sigma’_t x V’T _t$

-- $X’ = X + M’_t$ 

-- Calculate contrastive loss Ls on X’ by inference the model F and SSL model S $\rightarrow$ get gradient for $U_t,  \Sigma_t, VT _t$

-- Update the three matrices $\rightarrow$ For example: $U_{t+1} = U_t + \alpha * sign (U_{t} grad)$


\subsubsection{Are they directly applied to the input?} 
Yes the low-rank matrices are directly applied on input X

\subsubsection{Clarificaion: apply low-rank prompt on input X}

We describe the detail of how the low-rank prompt is applied on input X and fed to the convolutional architecture. It is not only the LoRA paper [24] using low-rank matrices. Prior literature [1] has shown that the low-rank matrices can be applied to convolutional neural networks for denoising.

[1] Yang, Yuzhe, et al. "Me-net: Towards effective adversarial robustness with matrix estimation." arXiv preprint arXiv:1905.11971 (2019).


\subsubsection{Compare low-rank prompts with CVP}
% As two low-rank matrices are involved (I'm supposing so, as details are missing), this evidently involves more learnable parameters and is thus susceptible to overfitting. So, the comparison to conv kernels is not fair. 
Thank the reviewer for pointing out this. We agree that the low-rank prompt induces more learnable parameters due to the decomposition of matrices. However, compared with VP, the number of learnable parameters within CVP and low-rank prompts are less than 1\% to 9\% parameters which are indeed light-weight. Therefore, we want to highlight both of these lightweight prompts have significant improvement on the performance.


\subsection{The corresponding figure in Appendix (Fig. 9), does not have any descriptive captions. It’s better not to give such figures if everything about the figure has to be inferred by the reader}

We are sorry for the missing details. We already added the full caption for Fig. 9 in our PDF.

\subsection{Line 266-271: Questions about SSL tasks}

Sorry for the confusion. The 'Standard' means the backbone model pre-trained on the source domain without adding SSL. Here in Table 7, the standard model is the ResNet50 pre-trained on ImageNet. We compare the adaptation performance of three SSL tasks with this standard model.

\subsection{Difference with 'contrastive' variation needs to be detailed}


In Table 7. we have a typo in the caption. The reported results are the average robust accuracy, not the average error rate. As the subparagraph 'Generalize CVP to other SSL tasks' in the Ablation study mentioned, our CVP improves robust accuracy for every severity level (from s1 to s5) on ImageNet-C when optimized for all three SSL tasks. We find contrastive learning can perform better than rotation prediction, and MAE has the best performance. 
We will add the details of SSL tasks in our later revision.

\subsection{How many variations of rotation prediction were used?}
We have four degrees for our rotation prediction tasks, including 0, 90, 180, 270.

\subsection{How much percentage of the images were masked in MAE?}
We setup 75 percent of the images to be masked in MAE.

\subsection{Is there any study by varying the mask percentage?}
We follow the default setting in [2] for setting up the mask percentage. We will add more study on the varying of the mask percentage for MAE. 

[2] He, Kaiming, et al. "Masked autoencoders are scalable vision learners." Proceedings of the IEEE/CVF conference on computer vision and pattern recognition. 2022.

- How long are these other SSL tasks trained? 
As our MLP model is small, the SSL tasks take only 1~2 hours for training.

- Generally Contrastive and MAE tasks require long training for better learning. Was this good practice followed?

Our SSL tasks only need to train once before doing the adaptation. Once the SSL has been trained, we can use this foradapting multiple target domains.



==> docs/rebuttal_figs.tex <==

% \begin{samepage}

\begin{figure}[h]{}
         \centering
         \includegraphics[width=0.6\linewidth]{figs/flow_cvp.png}
         \caption{}
         \label{fig:ssl_shortcut}
\end{figure}




% \subsection{number of learnable parameter}
% \begin{figure}[h]{}
%     \centering
%      \includegraphics[width=0.55\linewidth]{figs/new_acc_vs_param.png}
%     \caption{}
%     \label{fig:teaser}
% \end{figure}

% \begin{figure}[h]{}
%     \centering
%      \includegraphics[width=0.65\linewidth]{figs/unseen_loss_analysis.png}
%     \caption{}
%     \label{fig:teaser}
% \end{figure}



\begin{figure}[h]
\vspace{-5mm}
\centering
\scalebox{0.8}{
     \begin{subfigure}[b]{0.20\textwidth}
        \centering
         \includegraphics[width=\textwidth]{figs/new_acc_vs_param.png}
          \caption{Number of learnable parameters}
     \end{subfigure}
         \hfill
     \begin{subfigure}[b]{0.20\textwidth}
              \centering
         \includegraphics[width=\textwidth]{figs/unseen_loss_analysis.png}
         \caption{Blur Group}
     \end{subfigure}}
\caption{}
\label{fig:swd_violin}

\end{figure}



% \begin{figure}[h]{}
%          \centering
% \includegraphics[width=0.5\linewidth]{figs/ssl_shortcut_analysis.png}
%          \caption{add caption......}
%          \label{fig:ssl_shortcut}
% \end{figure}


\vspace{-5mm}

\begin{table}[h]
\small
\centering
\begin{adjustbox}{width=8in,center}
\begin{tabular}{lllllllllllllllll}
\hline
         & Gauss. & Shot  & Impulse & Defocus & Motion & Glass & Zoom  & Bright & Fog   & Snow  & Frost & Contr. & Elastic & JPEG  & Pixel. & Avg. \\
standard & 47.6    & 41.9 & 80.8   & 27.9   & 58.3  & 48.5 & 83.7 & 94.4      & 74.7 & 89.3 & 90.1 & 90.1    & 40.6   & 62.5 & 66.0    & 66.4     \\
VP       & 49.7    & 45.6 & 80.3   & 27.3   & 56.2  & 47.7 & 83.2 & 93.1      & 73.6 & 88.2 & 92.1 & 91.3    & 40.5   & 61.5 & 66.3    & 66.4     \\
CVP      & 50.2    & 46.0 & 82.1   & 28.9   & 58.8  & 49.1 & 85.6 & 94.5      & 75.6 & 89.4 & 92.3 & 92.3    & 41.5   & 63.5 & 63.5    & 67.8     \\ \hline
\end{tabular}
\end{adjustbox}
\caption{ViT Results}
\vspace{-5mm}
\end{table}


\begin{figure}
         \centering
\includegraphics[width=0.5\linewidth]{figs/ssl_shortcut_analysis.png}
         \caption{add caption......}
         \label{fig:ssl_shortcut}
\end{figure}
% \end{samepage}
